From Off-Policy to On-Policy: Enhancing GUI Agents via Bi-level Expert-to-Policy Assimilation

Vision-language models are increasingly deployed as computer-use agents (CUAs) that operate desktops and browsers. Top-performing CUAs are framework-based systems that decompose planning and execution, while end-to-end screenshot-to-action policies are easier to deploy but lag behind on benchmarks such as OSWorld-Verified. GUI datasets like OSWorld pose two bottlenecks: they expose only a few hundred interactive, verifiable tasks and environments, and expert trajectories must be gathered by interacting with these environments, making such data hard to scale. We therefore ask how reinforcement learning from verifiable rewards (RLVR) can best exploit a small pool of exist expert trajectories to train end-to-end policies. Naively mixing these off-policy traces into on-policy RLVR is brittle: even after format conversion, expert trajectories exhibit structural mismatch and distribution shift from the learner. We propose BEPA (Bi-Level Expert-to-Policy Assimilation), which turns static expert traces into policy-aligned guidance via self-rolled reachable trajectories under the base policy (LEVEL-1) and a per-task, dynamically updated cache used in RLVR (LEVEL-2). On OSWorld-Verified, BEPA improves UITARS1.5-7B success from 22.87% to 32.13% and raises a held-out split from 5.74% to 10.30%, with consistent gains on MMBench-GUI and Online-Mind2Web. Our code and data are available at: https://github.com/LEON-gittech/Verl_GUI.git

==> sections/table_and_fig/ablation.tex <==
\begin{table}[t]
\centering
\small
\setlength{\tabcolsep}{2.5pt}
\begin{tabular}{@{}l c c c c@{}}
\toprule
\textbf{Var.} & \textbf{Replacement} & \textbf{L1} & \textbf{L2} & \textbf{BEPA} \\
\midrule
\textbf{Overall (\%)} & 23.91 & 27.30 & 29.74 & 31.47 \\
\bottomrule
\end{tabular}
\caption{\textbf{Ablation on OSWorld-Verified.} Final overall performance.}
\label{tab:ablation_overall}
\end{table}


==> sections/table_and_fig/distgap.tex <==
\begin{table}[t]
\centering
\small
\setlength{\tabcolsep}{4pt}

% -------------------- (A) Token distribution stats --------------------
\begin{tabular}{@{}l r r@{}}
\toprule
\multicolumn{3}{c}{\textbf{(A) Token-Probability Distribution Gap}} \\
\midrule
\textbf{Method} &
$\boldsymbol{\Pr(p<0.2)}$ &
$\boldsymbol{JS(\cdot\,\|\,P_{\text{ref}})}\downarrow$ \\
\midrule
Converted             & 18.35\% & 0.1151 \\
LEVEL-1 (self-rolled) & 10.53\% & 0.1525 \\
After Cache Update    & 19.88\% & 0.0366 \\
\bottomrule
\end{tabular}

\vspace{6pt}

% -------------------- (B) Expert-task learning --------------------
\begin{tabular}{l c c c c}
\toprule
\multicolumn{5}{c}{\textbf{(B) Expert-Only Success Rate on $\mathcal{D}_E$ (\%)}} \\
\midrule
\textbf{Method} & \textbf{Ep1} & \textbf{Ep2} & \textbf{Ep3} & \textbf{Ep4} \\
\midrule
Replacement & 10.5 & 13.0 & 14.0 & 14.3 \\
LEVEL-1     & 12.0 & 17.0 & 18.5 & 19.0 \\
LEVEL-2     & 9.5  & 16.5 & 24.5 & 27.6 \\
BEPA        & 12.5 & 23.0 & 30.5 & 33.3 \\
\bottomrule
\end{tabular}

\caption{\textbf{Distribution alignment and off-policy learning.}
(A) Tail mass $\Pr(p<0.2)$ and Jensen--Shannon (JS) divergence to the on-policy reference distribution $P_{\text{ref}}$ (lower is closer). On-Policy's $P_{\text{ref}}$ is $26.95\%$.
(B) Success rate on expert-only-success tasks across epochs.}
\label{tab:distgap_expert_sr}
\end{table}

==> sections/table_and_fig/mmbench.tex <==
\begin{table*}[t]
\centering
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{l|cc|cc|cc|cc|cc|cc}
\toprule
\multirow{2}{*}{\textbf{Method}} & \multicolumn{2}{c|}{\textbf{L1-Easy}} & \multicolumn{2}{c|}{\textbf{L1-Medium}} & \multicolumn{2}{c|}{\textbf{L1-Hard}} & \multicolumn{2}{c|}{\textbf{L2 (Basic/Adv.)}} & \multicolumn{2}{c|}{\textbf{L3 (SR/EQA)}} & \multicolumn{2}{c}{\textbf{L4 (SR/EQA)}} \\
& Linux & Web & Linux & Web & Linux & Web & Linux & Web & Linux & Web & Linux & Web \\
\midrule
\rowcolor{categoryblue}
\multicolumn{13}{c}{\textbf{\textit{Proprietary Models}}} \\
GPT-4o & 62.38 & 58.51 & 59.70 & 54.98 & 52.42 & 50.83 & 1.05/1.02 & 3.23/2.92 & 6.83/4.35 & 1.94/1.53 & 3.50/2.41 & 2.13/0.10 \\
Claude-3.7 & 39.37 & 40.80 & 42.28 & 36.17 & 31.97 & 38.92 & 1.05/0.00 & 3.23/2.27 & 7.43/4.20 & 1.94/1.46 & 7.32/4.76 & 2.13/0.03 \\
Qwen-Max-VL & 69.91 & 69.46 & 66.90 & 64.59 & 65.80 & 65.34 & 53.93/30.10 & 74.84/58.77 & - & - & - & - \\
\midrule
\rowcolor{categoryblue}
\multicolumn{13}{c}{\textbf{\textit{Open-Source Models}}} \\
Aguvis-72B & - & - & - & - & - & - & 33.51/25.00 & 61.61/45.45 & 3.09/1.63 & 9.03/3.75 & 1.62/0.37 & - \\
Qwen2.5-VL-72B & 73.02 & 72.08 & 72.63 & 68.24 & 70.98 & 68.10 & 40.31/20.92 & 68.39/45.78 & 9.80/5.37 & 15.58/9.92 & 2.53/1.65 & - \\
InternVL3-72B & 79.16 & 81.18 & 79.88 & 78.67 & 76.19 & 78.11 & 59.16/41.33 & 90.65/65.91 & - & - & - & - \\
UI-TARS-72B-DPO & 35.16 & 35.33 & 37.14 & 31.55 & 24.19 & 19.94 & 68.59/51.53 & 88.06/68.51 & 30.31/18.91 & 10.32/6.94 & 7.46/5.87 & - \\
UI-TARS-1.5-7B & 84.03 & 85.12 & 84.07 & 81.34 & \textbf{95.43} & 92.17 & 67.02/40.31 & 87.74/61.36 & 26.51/18.65 & 12.26/6.98 & 4.95/3.98 & - \\
\midrule
\rowcolor{categoryblue}
\multicolumn{13}{c}{\textbf{\textit{Modular Agents}}} \\
\makecell[l]{GPT-4o$^\dagger$} & - & - & - & - & - & - & - & - & 16.13/8.69 & 23.23/16.69 & 3.60/2.51 & 4.26/0.61 \\
\makecell[l]{GPT-4o$^\ddagger$} & - & - & - & - & - & - & - & - & 20.23/11.12 & 22.58/14.65 & 5.58/3.82 & 4.26/0.68 \\
\midrule
\rowcolor{categoryblue}
\multicolumn{13}{c}{\textbf{\textit{UITARS1.5-7B+}}} \\
GRPO & 87.53 & 88.32 & 87.27 & 85.14 & 93.43 & 90.79 & 69.42/42.51 & 90.04/64.26 & 30.85/20.45 & 15.00/8.85 & 6.50/5.20 & 2.20/1.50 \\
LUFFY & 79.91 & 86.49 & 86.05 & 76.79 & 91.74 & 92.20 & 65.97/37.24 & 85.16/62.01 & 24.50/17.10 & 11.00/6.20 & 3.50/2.80 & - \\
\textbf{BEPA} (ours) & \textbf{91.53} & \textbf{93.22} & \textbf{90.87} & \textbf{89.84} & 94.89 & \textbf{94.57} & \textbf{70.82/44.31} & \textbf{91.94/66.16} & \textbf{35.50/24.10} & \textbf{18.50/11.20} & \textbf{8.80/7.80} & \textbf{3.50/2.80} \\
\bottomrule
\end{tabular}
\end{adjustbox}
\caption{\textbf{Performance on MMBench-GUI (Linux and Web domains)}. L1: GUI Content Understanding, L2: GUI Element Grounding (Basic/Advanced scores), L3: GUI Task Automation, L4: GUI Task Collaboration. For L3 and L4, we report Success Rate (SR) and Exact Question Answering (EQA) scores. All experiments use Max Step=15. $^\dagger$GPT-4o + UGround-V1-7B; $^\ddagger$GPT-4o + UI-TARS-1.5-7B.}
\label{tab:mmbench-gui}
\end{table*}
